Deep Reinforcement Learning for 6G AI-RAN: A Comprehensive Survey

The evolution toward sixth-generation (6G) networks is transforming the radio access network (RAN) into a programmable and intelligent control platform that must continuously adapt to heterogeneous services, dynamic environments, and competing performance objectives. Open Radio Access Network (O-RAN) provides the open interfaces, disaggregated architecture, and multi-timescale control loops needed to support this transformation, while deep reinforcement learning (DRL) offers a natural framework for optimizing sequential decisions under uncertainty. However, existing surveys either address artificial intelligence (AI) and machine learning (ML) in O-RAN broadly or focus on isolated DRL use cases, leaving a gap in the systematic connection between DRL methodology, O-RAN architecture, and operational deployment. To the best of our knowledge, this article presents the first dedicated and comprehensive survey of DRL for Open AI-RAN. We review the foundations of model-free, model-based, offline, safe, multi-agent, federated, and transfer learning, and provide an O-RAN-aware framework for formulating RAN control problems through states, observations, actions, rewards, constraints, and temporal structure. We classify DRL applications across radio resource management, mobility management, interference control, traffic steering, energy efficiency, network slicing, integrated sensing and communication, security, and massive MIMO. We further examine multi-agent and federated coordination, foundation models and agentic AI, trustworthy DRL, sim-to-real transfer, continual adaptation, resource-efficient inference, and reinforcement learning operations. Finally, we review experimental platforms, benchmarks, standards, and industry activities, and identify research directions toward sample-efficient, safe, scalable, interoperable, and deployable DRL control for 6G Open AI-RAN.

==> tables/sec10/sec10_table_benchmark_suite.tex <==
\begin{table*}[!t]
\centering
\caption{A minimal benchmark suite for DRL-based O-RAN. Each task should include reference configurations, seeds, baselines, and logging scripts.}
\label{tab:benchmark-suite}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{
|>{\raggedright\arraybackslash}m{0.155\textwidth}
|>{\raggedright\arraybackslash}m{0.175\textwidth}
|>{\raggedright\arraybackslash}m{0.190\textwidth}
|>{\raggedright\arraybackslash}m{0.185\textwidth}
|>{\raggedright\arraybackslash}m{0.260\textwidth}|}
\hline
\rowcolor[gray]{0.9}
\multicolumn{1}{|c|}{\parbox[c][6ex][c]{0.155\textwidth}{\centering \textbf{Task}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.175\textwidth}{\centering \textbf{Agent placement}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.190\textwidth}{\centering \textbf{Representative actions}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.185\textwidth}{\centering \textbf{Primary metrics}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.260\textwidth}{\centering \textbf{Stress tests}}} \\
\hline

Traffic steering & Near-RT xApp or non-RT-guided xApp & Target cell, handover bias, steering preference & Throughput, handover rate, mobility failure, fairness & Mobility bursts, load imbalance, stale measurements \\
\hline
Network slicing & Near-RT xApp with non-RT policy guidance & PRB share, scheduling weight, slice admission, slice scaling & SLA violation, per-slice throughput, latency, utilization & Sudden demand shift, mixed eMBB/URLLC/mMTC traffic \\
\hline
Scheduler reconfiguration & Near-RT xApp or dApp & Scheduler type, scheduler parameters, per-slice priority & Delay, buffer occupancy, packet delivery, fairness & Bursty traffic, mixed QoS classes, delayed rewards \\
\hline
Resource allocation & xApp or dApp & Power, MCS, resource blocks, beam or link selection & Spectral efficiency, interference, energy per bit & Channel shift, cell-edge users, action feasibility limits \\
\hline
Energy saving & rApp plus xApp execution & Sleep mode, carrier activation, antenna activation, functional split & Energy, capacity, wake-up latency, SLA margin & Diurnal traffic, emergency load, wake-up delay \\
\hline
Security and robustness & xApp, rApp, or monitor & Mitigation action, robust policy update, fallback trigger & SLA under attack, recovery time, false alarm rate & Jamming, telemetry poisoning, evasion perturbations \\
\hline
\end{tabular}
\end{table*}


==> tables/sec10/sec10_table_reporting_checklist.tex <==
\begin{table*}[!t]
\caption{Minimum reporting checklist for DRL-based O-RAN experiments.}
\label{tab:reporting-checklist}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|>{\raggedright\arraybackslash}p{0.12\textwidth}|>{\raggedright\arraybackslash}p{0.85\textwidth}|}
\hline
\rowcolor[gray]{0.9}
\textbf{Category} & \textbf{Items to report} \\
\hline
Deployment context & Agent type and placement (xApp, rApp, dApp, etc.), RIC implementation, control-loop timescale, interface assumptions, action-delivery mechanism \\
\hline
Learning formulation & Observation/state, action, reward, constraints, discount factor, episode or continuing-task definition, feasibility handling, delay modeling \\
\hline
Algorithm details & Algorithm, policy/value architecture, optimizer, learning rate, batch size, replay buffer, exploration, update frequency, number of training steps, etc. \\
\hline
Environment & Simulator/emulator/testbed, channel model, traffic model, mobility model, topology, slice configuration, user distribution, hardware and software versions \\
\hline
Baselines & Classical baselines, optimization or model-based baselines, DRL baselines, hyperparameters, ablations, baseline tuning procedure \\
\hline
Metrics & Network KPIs, learning curves, convergence, sample efficiency, training cost, inference latency, action latency, safety violations, fairness, robustness \\
\hline
Artifacts & Code, configuration files, container images, trained models, datasets or traces, seed lists, scripts for figure generation \\
\hline
Robustness & Evaluation under distribution shift, noisy observations, delayed measurements, unseen traffic, mobility bursts, failures, and adversarial perturbations \\
\hline
\end{tabular}
\end{table*}

==> tables/sec11/sec11_table_ecosystem.tex <==
\begin{table*}[!t]
\centering
\caption{Representative open-source and research ecosystem components for DRL-based O-RAN.}
\label{tab:ecosystem}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.18}
\begin{tabular}{|>{\raggedright\arraybackslash}m{0.175\textwidth}|>{\raggedright\arraybackslash}m{0.225\textwidth}|>{\raggedright\arraybackslash}m{0.315\textwidth}|>{\raggedright\arraybackslash}m{0.250\textwidth}|}
\hline
\rowcolor[gray]{0.9}
\multicolumn{1}{|l|}{\parbox[c][6ex][c]{0.175\textwidth}{\raggedright \textbf{Layer}}} &
\multicolumn{1}{l|}{\parbox[c][6ex][c]{0.225\textwidth}{\raggedright \textbf{Examples}}} &
\multicolumn{1}{l|}{\parbox[c][6ex][c]{0.315\textwidth}{\raggedright \textbf{Role in DRL-for-O-RAN}}} &
\multicolumn{1}{l|}{\parbox[c][6ex][c]{0.250\textwidth}{\raggedright \textbf{Adoption challenge}}} \\
\hline

RAN stack & srsRAN, OpenAirInterface & Generates protocol behavior, telemetry, and controllable RAN functions & Need stable O-RAN agents, service-model support, and reproducible configuration \\
\hline
Near-RT RIC & OSC Near-RT RIC, ONF SD-RAN, FlexRIC & Hosts xApps, manages E2 interaction, provides platform services & Need portable xApps and consistent APIs across RIC implementations \\
\hline
Non-RT RIC and SMO & OSC Non-RT RIC, ONAP, OSM & Hosts rApps, data services, policy generation, lifecycle management & Need integration of model catalogs, A1-ML, and RLOps workflows \\
\hline
Experimentation framework & ColO-RAN, OpenRAN Gym, ns-O-RAN, OAIC & Provides training, evaluation, and interface-aware experimentation & Need shared benchmark tasks and public trajectory datasets \\
\hline
Large-scale testbed & Colosseum, POWDER, COSMOS, AERPAW, SLICES & Adds wireless realism, scale, mobility, or outdoor experimentation & Need easier repeatability and standardized experiment descriptions \\
\hline
\end{tabular}
\end{table*}

==> tables/sec11/sec11_table_oran_drl_specs.tex <==
\begin{table*}[!t]
\centering
\caption{O-RAN specification elements that constrain or enable DRL-based controllers.}
\label{tab:oran-drl-specs}
\scriptsize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{
|>{\raggedright\arraybackslash}m{0.110\textwidth}
|>{\raggedright\arraybackslash}m{0.125\textwidth}
|>{\raggedright\arraybackslash}m{0.190\textwidth}
|>{\raggedright\arraybackslash}m{0.200\textwidth}
|>{\raggedright\arraybackslash}m{0.290\textwidth}|}
\hline
\rowcolor[gray]{0.9}
\multicolumn{1}{|c|}{\parbox[c][6ex][c]{0.110\textwidth}{\centering \textbf{Element}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.125\textwidth}{\centering \textbf{Primary host}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.190\textwidth}{\centering \textbf{DRL relevance}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.220\textwidth}{\centering \textbf{Typical control role}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.290\textwidth}{\centering \textbf{Open issue for DRL adoption}}} \\
\hline

R1 and SMO data services & Non-RT RIC / SMO & Access to aggregated data, analytics, and lifecycle services & Offline training, long-horizon optimization, policy generation & Need portable data schemas and model-provenance tracking for rApps \\
\hline
A1-P & Non-RT RIC to Near-RT RIC & High-level policy guidance & Hierarchical DRL, policy shaping, objective constraints & Need explicit mapping from learned policies to enforceable, testable A1 policy statements \\
\hline
A1-EI & Non-RT RIC to Near-RT RIC & External context and predictions & Forecast-aware xApps and multi-timescale control & Need quality indicators for forecasts and stale enrichment information \\
\hline
A1-ML & Non-RT RIC to Near-RT RIC & Model distribution and management & Model update, versioning, rollback, and lifecycle control & Need mature procedures for DRL-specific model metadata and safe rollout \\
\hline
E2SM KPM & Near-RT RIC to E2 nodes & Measurement stream for state construction & Observation path for xApps & Need benchmark-level agreement on KPM selection, granularity, delay, and missing data \\
\hline
E2SM RC & Near-RT RIC to E2 nodes & RAN control primitives & Action path for xApps & Need action feasibility, conflict handling, and safety envelopes for learned policies \\
\hline
O1 and O2 & SMO / O-Cloud & Management, telemetry, workload placement & Offline data collection, model deployment, infrastructure adaptation & Need tighter coupling between model placement, inference latency, and orchestration policy \\
\hline
\end{tabular}
\end{table*}


==> tables/sec11/sec11_table_regulatory_policy.tex <==
\begin{table*}[!t]
\centering
\caption{Mapping regulatory and policy concerns to technical mechanisms for DRL-based O-RAN.}
\label{tab:reg}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|>{\centering\arraybackslash}m{0.1\textwidth}|m{0.47\textwidth}|m{0.415\textwidth}|}
\hline
\rowcolor[gray]{0.9}
\multicolumn{1}{|c|}{\parbox[c][6ex][c]{0.1\textwidth}{\centering \textbf{Concern}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.47\textwidth}{\centering \textbf{Technical mechanism}}} &
\multicolumn{1}{c|}{\parbox[c][6ex][c]{0.415\textwidth}{\centering \textbf{Evidence to report or certify}}} \\
\hline

Accountability & Model provenance, action logs, policy versioning, rollback records & Which model acted, which inputs it used, which action was delivered, and what fallback was available \\
\hline
Auditability & Training-data documentation, validation scenarios, objective and constraint declarations & Dataset description, reward and constraint definition, validation coverage, SLA thresholds \\
\hline
Explainability & Feature attribution, surrogate models, reward decomposition, counterfactual analysis & Explanation reports for representative decisions and failure cases \\
\hline
Safety & Constrained RL, runtime shielding, action projection, fallback controllers, conflict mitigation & Bound on unsafe actions, constraint-violation rate, recovery time, fallback success rate \\
\hline
Privacy & Data minimization, anonymization, federated RL, secure aggregation, differential privacy & Description of telemetry use, storage policy, privacy protection mechanism, leakage assessment \\
\hline
Interoperability & Standard service models, portable descriptors, interface conformance testing & E2/A1/R1/O1 assumptions, supported RIC platforms, packaging and descriptor validation \\
\hline
\end{tabular}
\end{table*}

